Towards Hierarchical Importance Attribution: Explaining Compositional Semantics for Neural Sequence Models

The impressive performance of neural networks on natural language processing tasks attributes to their ability to model complicated word and phrase compositions. To explain how the model handles semantic compositions, we study hierarchical explanation of neural network predictions. We identify non-additivity and context independent importance attributions within hierarchies as two desirable properties for highlighting word and phrase compositions. We show some prior efforts on hierarchical explanations, e.g. contextual decomposition, do not satisfy the desired properties mathematically, leading to inconsistent explanation quality in different models. In this paper, we start by proposing a formal and general way to quantify the importance of each word and phrase. Following the formulation, we propose Sampling and Contextual Decomposition (SCD) algorithm and Sampling and Occlusion (SOC) algorithm. Human and metrics evaluation on both LSTM models and BERT Transformer models on multiple datasets show that our algorithms outperform prior hierarchical explanation algorithms. Our algorithms help to visualize semantic composition captured by models, extract classification rules and improve human trust of models. Project page: https://inklab.usc.edu/hiexpl/

==> method__old.tex <==
\section{Methodology}

% \xiang{need 2-3 sentences to overview this section.}

Despite the empirical success of CD and ACD, no prior works analyze what common properties a score attribution mechanism should satisfy to generate hierarchical explanations that reveal compositional semantics formed between phrases. 


\subsection{Properties of Attribution for Hierarchical Explanation}
Here we identify two properties that an attribution method should satisfy to generate informative hierarchical explanations.

\textbf{Non-additivity} As suggested by both CD and ACD, the algorithm should be able to attribute contribution scores for phrases $\phi(\rvp,\rvx)$ that do not necessarily equal to the sum of the scores of component words.

\textbf{Context Independence} 
% \xisendone{Please discuss with me if you think this part is confusing...}
Intuitively, in order to study the contribution from the composition between two phrases, a simple way is to study the sum of the contributions of two phrases $\rvp_1$ and $\rvp_2$ independent of each other, and study the contribution of the combined phrase, then observe the discrepancy between the two. This follows the measurement of surplus by combing two groups of players in game theory~\citep{driessen2013cooperative} if we treat each word as a player and the phrase as a set of players. 
Formally, if we are interested in the compositional effect of two phrases $\rvp$ and $\rvp^\prime$ in an input sentence $\rvx$, for any input sentence $\hat{\rvx}$ where only $\rvp^\prime$ is replaced to another phrase, we expect the attribution for $\rvp$ remains the same, i.e., $\phi(\rvp, \rvx) = \phi(\rvp, \hat{\rvx})$. In our hierarchical explanation setting, we are interested in the compositional effect of any two phrases in $\rvx$. Therefore, we expect the attribution $\phi(\rvp, \rvx) = \phi(\rvp, \hat{\rvx})$ given the $\rvp$ in two different contexts $\rvx$ and $\hat{\rvx}$. In this case, the notation $\phi(\rvp, \rvx)$ simplifies to $\phi^g(\rvp)$.


%In the view of cooperative game theory, the set of players maps to a value with a characteristic function $v(\cdot)$, and the surplus of forming a coalition of players is measured with dividends. , and expect the $\phi(\rvp)$ represent the value $v(\rvp)$ of the phrase. The discrepancy $\phi(\rvp_1\rvp_2) - \phi(\rvp_1) - \phi(\rvp_2)$ represent the sum of the harsanyi dividends between every subset of words in two phrases. 

%To represent how the semantics build up from atomic words, we expect the score attribution of a phrase is 

%\xiang{to be more convincing: (1) use math formulation to explain issues; (2) add case study or analysis evidences to support the claims.}
\textbf{Limitations of CD and ACD} Unfortunately, while CD and ACD try to construct decomposition so that $\beta$ terms represent the contributions solely from a given a phrase, they do not satisfy the context independence property mathematically. %The decomposition in Eq.~\ref{eq:cd} makes the explanations of contextual decomposition of \cite{murdoch2018beyond} deviate from the goal of studying the contributions solely made by a given phrase as claimed. 
For CD, we see the computation of $\mathbf{\beta}$ involves the $\mathbf{\gamma}$ term of a specific input sentence in Eq.~\ref{eq:cd}. Similarly, for ACD, the decomposition of the bias term involves the $\mathbf{\gamma}$ terms of a specific input sentence. As a result, the $\beta$ terms computed by both algorithms depend on the context of the phrase $\rvp$.
%\junyi{if I understand correctly, here the involvement refers that the $\mathbf{\beta}_t^i$ requires $\mathbf{\gamma}_t^{i_x}$ which actually is the $\mathbf{\gamma}_{t-1}^h$ ? Maybe can keep the $\mathbf{\gamma}$ to the original form in terms of (t-1) for the formulations, and point out these superscript/subscript in the sentence, so we could find out the involvement from (6) easily}
%Actually, Eq.~\ref{eq:cd} is similar in its form to Shapley Values~\citep{shapley1997value} of two terms as suggested by authors, while Shapley Values are known to be specific to other input variables in the given example.
Regarding the decomposition of activation functions, the decomposition $\beta^\prime=\sigma(\beta)$ in ACD seems plausible, which does not involve $\mathbf{\gamma}$ for computing $\mathbf{\beta}$ terms. However, in case every activation is decomposed in this way and suppose the bias terms are merged into $\mathbf{\beta}$, the algorithm is equivalent to feeding only the phrase $\rvp$ into the classifier with all other input masked as zero. 
%It makes the decomposition shares the same vulnerability as taking the model prediction scores on phrase fragments as explanations. 
Empirical results show unreliable explanation quality of both algorithms in some models. %It assume  obtaining the contribution score by directly feeding a phrase fragment to the model, which assume evaluate the model on inputs that are significantly out of the normal data distribution. 

%In the next section, we formally define individual contributions of phrases, and define mathematically \emph{what to be explained} by our explanation algorithms. In accordance with our formulation, we propose a new explanation algorithm, and show that contextual decomposition algorithms also fit into our formulation with moderate modification.

% Unfortunately, without a formal definition of individual contributions, the decomposition in Eqs.~\ref{eq:cd} and \ref{eq:cd_2019} are heuristic and lack of justification; the performance of algorithms is also inconsistent over different models. For example,~\citet{singh2018hierarchical} find that the original contextual decomposition does not work well on deeper CNN models. More importantly, lack of a formal definition of individual contributions, it is hard to explain what property the algorithm explains about the model.

%where we see that $\mathbf{\beta}^\prime$ is no longer related to $\mathbf{\gamma}$. 
%We also show in our experiments that the decomposition can be further improved. 

% \subsection{Transformer Models}
% The Transformer~\cite{vaswani2017attention} is a model architecture that models sequences with only attentions. The attention operation computes a weighted sum of input values $V$, where the weights are computed by the function of query vectors $Q$ and key vectors $K$. 
% \begin{equation}
%     \label{eq:transformer}
%     Attn(Q,K,V) = softmax(\frac{QK^T}{\sqrt{d_k}})V
% \end{equation}
% where $d_k$ is the dimension of the key vectors. 

% The transformer encoder consists of self-attention modules, where $Q$, $K$, $V$ are all the output of the previous attention layer, or the word vectors for the first layer. There is a feed forward layer with non-linear activation, and a layer-normalization layer after each attention layer. 

%\junyi {this paragraph could be expand to an individual sub-section of the challenge and solution for applying these properties?}
To this end, we identify the key challenge of the hierarchical explanation problem is to find out a way to quantify the contributions of individual words and phrases which satisfy non-additivity and context independence. 
We note that the context independence property implies we study hierarchical explanation as a global explanation problem~\citep{guidotti2018survey}. Compared with local explanation algorithms, global explanation algorithms are less studied for explaining individual predictions~\citep{poerner2018evaluating}, because they reveal the average behavior of models. However, with a hierarchical organization, we show global explanations are also powerful at explaining individual predictions, achieving better human evaluation scores and could explain compositional semantics where local explanation algorithms such as additive feature attribution algorithms totally fail. Moreover, we note that the use of explanation algorithms is not exclusive; we may apply explanation algorithms of different categories to make a more holistic explanation of model predictions.

\begin{figure}
\vspace{-0.5cm}
    \centering
    \includegraphics[width=\textwidth]{figs/fig_arch2.jpeg}
    \vspace{-0.5cm}
    \caption{(Left) Illustration of the CD and SCD at calculating the decomposition for $\rvh=\sigma(\beta + \gamma)$. Red lines indicate computation that make CD explanations dependent on the words outside the give phrase. (Right) Illustration of the sampling step $\rvx_\delta \sim p(\rvx_\delta | \rvx_{-\delta})$ for calculating the contribution of the word \textit{very} in SOC and SCD.}
    \label{fig:method_fig}
\end{figure}


\subsection{Context-Independent Individual Contribution}
Given a phrase $\rvp:=\rvx_{i:j}$ appearing in a specific input $\rvx_{1:T}$, we first relax our setting and define the contribution of a phrase independent of $N$ words adjacent to it. The \emph{N-context independent contribution} is defined as the output difference after masking the phrase $\rvp$, marginalized over all possible neighboring $N$ words $\rvx_\delta$ around $\rvp$ in the input $\rvx$. For an intuitive example, to evaluate the context independent contribution up to one word of \emph{very} in the sentence \emph{The film is very interesting} in a sentiment analysis model, we sample some possible adjacent words before and after the word \emph{very}, and observe the prediction difference after some practice of masking the word \emph{very}. We illustrate the process in Figure~\ref{fig:method_fig} (Right). The process is formally written as,
\begin{equation}
\label{eq:pg}
    \phi(\mathbf{p},\mathbf{x}) = \E_{\mathbf{x}_\delta }[s(\mathbf{x_{- \delta}}, \mathbf{x}_\delta) - s(\mathbf{x_{-\delta} \backslash \mathbf{p}}, \mathbf{x}_\delta)]
\end{equation}
\junyidone{the later term should be $s(\mathbf{x_{-\delta} \backslash \mathbf{p}}, \mathbf{x}_\delta)$ ? $\mathbf{p}$ is not in $\delta$ according to your description}

where $\rvx_{-\delta}$ is the notation for the input $\rvx$ after removing $N$ neighboring words of the phrase $\rvp$;  $s(\rvx_{-\delta}, \rvx_\delta)$ denotes model prediction score after replacing the neighboring words in the given input with sampled ones $\rvx_\delta$. $\rvx_\delta$ is sampled from a distribution $p(\rvx_\delta | \rvx_{-\delta})$, which is conditioned on the phrase $\rvp$ and the words outside the neighboring $N$ words. $\rvx \backslash \rvp$ denotes the masking operation on the phrase $\rvp$, which depends on the specific explanation algorithms instantiated from the formulation.

We define the \emph{individual contribution} of a phrase $\rvp$ when the size of the neighborhood $N$ is sufficiently large. The individual contribution can be equivalently written as,
\begin{equation}
    \label{eq:ces_nlp}
    \phi^g(\rvp) = \E_\mathbf{x}[s(\rvx) - s(\rvx\backslash \rvp) | \rvp \subseteq \rvx].
\end{equation}

%The proposed individual contribution is inspired by Accumulated Local Effect~\citep{apley2016visualizing}. 
Calculating both Eqs.~\ref{eq:pg} and~\ref{eq:ces_nlp} requires integrating over all possible inputs which contain the phrase $\mathbf{p}$. While it is natural to directly approximate the expectation by sampling from the training data, we find it common that a phrase occur sparsely in the corpus. Therefore, we approximate the expectation by sampling from a trained language model on the training set\junyidone{can call this a language model? NN is too vague} which models a smoothed distribution of $p(\rvx_\delta | \rvx_{-\delta})$. %The individual contributions in Eq.~\ref{eq:ces_nlp} is then approximated by enlarging the size of the neighborhood region $N$.
In practice, all our explanation algorithms implements $N$-context independent contributions following Eq.~\ref{eq:pg}, where the size of the neighborhood $N$ is a parameter to be specified.


% \xiang{I think we need better transition from above part to the following two subsections on the two algorithms.}

% \xiang{A better flow to arrange Secs 3.2, 3.3 will be: 1. extending ACD algorithm based on your new formulation of individual, and discuss the potential issues with such algorithm; 2. motivate and transit to another new algorithm based on OC idea.}

\subsection{Sampling and Contextual Decomposition Algorithm}

In CD, the property of context independence is comprised at the decomposition of activation functions. 
We fit the contextual decomposition method into our formulations by modifying the activation decomposition step in CD, and propose Sampling and Contextual Decomposition (SCD) algorithm. SCD is a layer-wise application of our formulation. Given the output $h$ of a hidden layer, which is already decomposed into $\beta$ + $\gamma$, we decompose the activation value $\sigma(h)$ as $\beta^\prime + \gamma^\prime$, where,
\begin{equation}
    \label{eq:pgcd}
    \begin{split}
            \beta^\prime = \E_{\gamma}[\sigma(\beta + \gamma) - \sigma(\gamma)] &= \E_{h}[\sigma(h) - \sigma(h-\beta)],
    \end{split}
\end{equation}
\ie, $\beta^\prime$ is defined as the expected difference between the activation values, integrated over all the possible $\gamma$ given $\beta$. Eq.~\ref{eq:pgcd} follows the formulation in Eq.~\ref{eq:ces_nlp}, where the masking operation is implemented with calculating $\sigma(h-\beta)$. %Similar to the SOC algorithm, SCD also requires sampling the neighborhood region of the phrase $\mathbf{p}$ given a specific input example $\mathbf{x}$.

The algorithm first generate a set of samples $\mathcal{S}$ with a trained language model. We pretrain a LSTM language model from two directions. For sampling, we mask the words that are not conditioned in $p(\rvx_\delta | \rvx_{-\delta})$. Some other sampling options include performing gibbs sampling from a masked language model~\citep{wang2019bert}. In practice, for each sample in $\mathcal{S}$, the algorithm records the input of the $i$-th non-linear activation function to obtain a sample set $\mathcal{S}_h^{(i)}$. During the explanation, the decomposition of the $i$-th non-linear activation function is calculated as,
\begin{equation}
    \label{eq:pgcd_sample}
    \beta^\prime = \frac{1}{|\mathcal{S}_h^{(i)}|} \sum_{h\in \mathcal{S}_h^{(i)}}[\sigma(h) - \sigma(h-\beta)].
\end{equation}
%Our decomposition is a generalization of CD and ACD. The decomposition in Eq.~\ref{eq:cd} is equivalent to having $h=\beta$ and that of the input example itself in the sample set\junyi{?}. Similarly, the decomposition in Eq.~\ref{eq:cd_2019} is equivalent to having only $h=\beta$ in the sample set. \junyi{to give more intuition to reader, add practical result of this equivalent, like, size of neighbourhood range equals 0}

Some neural models such as Transformers involve operations that normalize over different dimensions of a vectors, e.g. softmax functions and layer normalization operations. We observe improved performance by not decomposing the normalizer of these terms when the phrase $\rvp$ is shorter than a threshold, assuming that the impact of $\mathbf{p}$ to the normalizer can be ignored. Besides, for element-wise multiplication in LSTM models, we treat them in the same way as other non-linear operations and decompose them as Eq.~\ref{eq:pgcd}. 

% Transformers~\citep{vaswani2017attention} model a sentence with attention between words. The attention operation computes a weighted sum of input values $V$, where the weights are computed with query vectors $Q$ and key vectors $K$. 
% \begin{equation}
%     \label{eq:transformer}
%     Attn(Q,K,V) = softmax(\frac{QK^T}{\sqrt{d_k}})V
% \end{equation}
% where $d_k$ is the dimension of the key vector. During the decomposition, we only decompose the term $V$, while treating the weight term as model parameters.

% Layer normalization is another non-linear operation in Transformers. The operation normalizes the input vector $h$ to a fixed mean and variance over its dimensions. When $|\mathbf{p}| \ll |\mathbf{x}|$, the impact of $\mathbf{p}$ to the mean and variance can be ignored. We observe improved performance by not decomposing these operations when $\mathbf{p}$ is shorter than a threshold, set as 20\% of the input sequence length.

% The algorithm keeps the contribution of the bias term $b$ as $\zeta=\sigma(b)$ temporally before the element-wise multiplication, as shown in Eq.~\ref{eq:cd}. %Following the original CD algorithm, we add the sample $h=\beta$ to the sample set $\mathcal{S}_h$ and let it take up half of the weight, where we see improved performance.

\subsection{Sampling and Occlusion Algorithm}
While SCD allows to design different decomposition schemes for different non-linear operations, a simpler approach is to directly approximate the $N$-context independent contribution in Eq.~\ref{eq:pg}, where the masking operation $\rvx \backslash \rvp$ is implemented by replacing the phrase $\rvp$ with padding tokens at the input sequence. 
%While SCD allows to design different decomposition schemes for different non-linear operations, 


We propose a simple and model-agnostic explanation algorithm, Sampling and Occlusion (SOC). % input occlusion, similar to those implemented in various input occlusion based local explanation methods. \xiang{This is too vague to me so please elaborate on (1) high-level idea of this algorithm; (2) more details on how to adapt from prior version to this new version.} Therefore, the algorithm can be viewed as a generalization of input perturbation based explanation algorithms. 
Similar to SCD, the algorithm samples from a trained language model $p(\rvx_\delta | \rvx_{-\delta})$ to obtain a set of neighboring word replacement $\mathcal{S}$. For each replacement $x_\delta \in \mathcal{S}$, Sampling and Occlusion computes the model prediction differences $s(\mathbf{x_{- \delta}}, \mathbf{x}_\delta) - s(\mathbf{x_{-\delta}}\backslash \mathbf{p}, \mathbf{x}_\delta )$ after occluding the phrase $\mathbf{p}$. 
%The masking operation $\mathbf{x}\backslash \mathbf{p}$ is implemented by replacing the phrase $\rvp$ with padding tokens, following input occlusion algorithms~\citep{li2016understanding}. 
The contribution $\phi(\rvp, \rvx)$ is then calculated as the average prediction differences. Formally, the algorithm calculates,
\begin{equation}
    \label{eq:soc}
    \begin{split}
        \phi(\mathbf{p},\mathbf{x}) = \frac{1}{|\mathcal{S}|}\sum_{\mathbf{\mathbf{x}_\delta} \in \mathcal{S}}[s(\mathbf{x_{- \delta}}, \mathbf{x}_\delta) - s(\mathbf{x_{-\delta}}\backslash \mathbf{p}, \mathbf{x}_\delta )].
    \end{split}
\end{equation}
Sampling and Occlusion is advant

==> prelim_old.tex <==
\section{Background}
\label{sec:prelim}
\subsection{Post-hoc Explanations of Neural Sequence Model Predictions}
% \xiang{Suggested structure for this section: 
% 1. notations and formal definition for ``RNNs" and ``post-hoc explanation" (from words, to phrases, to hierarchical).
% 2. brief introduction of the line of work on CD and ACD (try to follow unified notations in your whole paper); 
% 3. detailed discussion of the issues with ACD line of work.}

% \subsection{Neural Architectures For Text Modeling}
We consider a sequence of low-dimensional word embeddings $\rvx_{1:T} := (\rvx_1, \rvx_2, ...,\rvx_T$), or denoted as $\rvx$ for brevity, as the input to a neural sequence model, such as standard RNNs, LSTM and Transformers~\citep{vaswani2017attention}. 
% For example, Long Short Term Memory networks (LSTM)~\citep{hochreiter1997long} iteratively update a hidden state vector $\rvh_t\in\R^{d_h}$ and a cell state vector $\rvc_t\in\R^{d_h}$ at each time-step $t$.
% \begin{equation}
% \label{eq:lstm}
%      \rvc_t, \rvh_t = {\rm LSTM}(\rvx_t, \rvc_{t-1}, \rvh_{t-1})
% \end{equation}
These neural models extract latent, compositional representations from the input sequence $\rvx$, and feed hidden state vectors $\rvh_{1:T}$ to a prediction layer to generate output in the label space (\eg, sentiment polarity of a sentence). 
% To obtain a prediction from the representations of the input sequence $\rvx$, we map the extracted features, usually the final hidden state vector $\rvh_T$ for LSTMs to the label space. 
For LSTM, we uses the last hidden state $\rvh_{T}$ to give unnormalized prediction scores $s(\rvx)\in\R^{d_c}$ over $d_c$ label classes as follows.
\begin{equation}
\label{eq:projection}
    s(\rvx) = \mW_l\rvh_T,
\end{equation}
where $\mW_l\in\R^{d_c \times d_h}$ is a trainable weight matrix. 
For Transformers, the hidden state corresponding to the ``[CLS]" token at the final layer is fed to the prediction layer to generate scores $s(\rvx)$.
% Other successful architectures include Transformers~\citep{vaswani2017attention}, which model the input sequence with stacked layer of attentions. 
% Both architectures are powerful for modeling text data, especially when pretrained on large corpora~\citep{peters2018deep,devlin2018bert}.

% \xiang{do we need the below paragraph on details of Transformer?}
% Transformers~\citep{vaswani2017attention} are another powerful architecture to model text data. The main building block is the attention modules, which computes a weighted sum of input vectors at each layer. Given input value matrix $V\in\R^{T \times d_h}$, the model weights are computed with query vectors $Q\in\R^{T \times d_h}$ and key vectors $K\in\R^{T \times d_h}$. 
% \begin{equation}
%     \label{eq:transformer}
%     Attn(Q,K,V) = softmax(\frac{QK^T}{\sqrt{d_h}})V
% \end{equation}
% The attention layers are stacked in multiple layers with residual connections. To map the feature vectors to the label space,  Transformers use the representation at the final layer of a special token as the input for a linear layer, while LSTM networks usually use the final hidden state $\rvh_T$. Both architectures are powerful for modeling text data, especially when pretrained on large corpora~\citep{devlin2018bert, peters2018deep}.




% \subsection{Post-hoc Explanations of Neural Network Predictions}
% However, despite these deep models have achieved impressive results on many text prediction tasks, it is hard to interpret the model predictions. Researchers study post-hoc explanation algorithms to interpret model predictions with the trained model fixed.
Towards post-hoc explanation of $s(\rvx)$, a notable line of work, \textbf{additive word-level explanation methods}~\citep{lime, shrikumar2017learning, sundararajan2017axiomatic}, measures word-level contribution to the model prediction $s(\rvx)$ by attributing a contribution score $\phi(\rvx_i,\rvx)$ to each word in the input sequence $\rvx_i\in \rvx$.
Such additive attribution methods are related to Shapley Values~\citep{shapley1997value} and thus can be proven to enjoy good properties like having unique solution of a ``fair" attribution\citep{lundberg2017unified}.
However, the additive assumption hinders these methods from explaining the complex interactions between words and compositional semantics in a sentence (\eg, modeling negation, transition, and emphasis in sentiment classification).

% \textbf{Word-level Local Explanations of Predictions} Most prior work has focused on word-level contribution measure for specific predictions. The explanations are called local, as the score of a word is specific to the specific input example $\rvx^0$. 
% For a given input, additive word-level explanation algorithms~\citep{lime, shrikumar2017learning, sundararajan2017axiomatic} divide the contribution of the model prediction score $s(\rvx)$ to each input word $\rvx_i\in \rvx$ by assigning a contribution score $\phi(\rvx_i,\rvx)$.
% ~\citet{lundberg2017unified} provide a unified view of additive feature attribution algorithms with Shapley Values~\citep{shapley1997value}, which is proven as a unique solution for a ``fair'' attribution, which satisfies several mathematically properties. 
% However, due to the additive nature of contribution scores, the algorithms do not explain the interactions between words and compositional semantics such as stress and negation that the model has captured.


\subsection{Hierarchical Explanations via Contextual Decomposition}
\xiang{I move the last paragraph in Sec 2.1 to here and hope you can integrate and simplify this part.}
% \textbf{Phrase-level and Hierarchical Explanations} 
To handle the limitation of additive word level explanation algorithms,~\cite{murdoch2018beyond} study non-additive phrase level contribution measure, and propose the contextual decomposition (CD) algorithm. Given a specific input $\rvx^0$ and a phrase $\rvp=\rvx^0_{i:j}$, the algorithm attribute an contribution score $\phi(\rvp,\rvx^0)$ for the phrase, where the score usually do not equal to the sum of the scores of its component words.~\cite{singh2018hierarchical} generalize the algorithm to other family of networks, and propose agglomerative contextual decomposition algorithm (ACD). The algorithm generates a hierarchical layout of explanations automatically, capturing meaningful phrase interactions while displaying a sufficiently small subset of all possible phrases to maintain simplicity of explanations. Phrase level and hierarchical explanations are shown successful in visualizing complicated semantics captured by neural networks such as stress and negation, finding positive segment in negative sentences, and efficiently mining phrase level classification patterns. 

%Contextual decomposition (CD) algorithms~\citep{murdoch2018beyond} study phrase-level contribution attributions. %where the attribution usually do not satisfy $\phi(\rvp, x^0)=\sum_{t\in[i,j]}\phi(x_t)$.

%Given a sequence of words $\rvx_1,\rvx_2,...,\rvx_T$ and a phrase $\rvp=\rvx_{i...j}$ in the input, the algorithms assign an importance or contribution score $\phi(\rvp)$ for the phrase $\rvp$. While contextual decomp

%We briefly discuss some relevant explanation algorithms. Given a phrase $\rvp=\rvx_{i..j}$ \xiang{explain this notation?} in an input word sequence $\rvx_{1..T}$, an explanation algorithm attribute a contribution score $\phi(\rvp)$ for the phrase $\rvp$. The explanations are known as local explanations~\citep{guidotti2018survey} if the attribution is specific to the given input example $\rvx_{1..T}$.

% \xiang{I'm actually not quite sure if we need to introduce this line of work as they're not our focus.}
% \textbf{Input Occlusion Algorithm} Input occlusion algorithm is an example of local explanation algorithms. The algorithm computes the contribution of the phrase $\phi(\rvp, \rvx)$ by observing the prediction difference after replacing the phrase $\rvp$ with reference padding values~\citep{li2016understanding}, or removal~\citep{kadar2017representation}.
% \begin{equation}
%     \phi(\rvp, \rvx) = s(\rvx) - s(\rvx\backslash\rvp)
% \end{equation}
% where $s(\cdot)$ is the neural network prediction function. Intuitively, the prediction difference depends on the context of the phrase $\rvp$.

%\subsection{Contextual Decomposition Algorithm}
% \textbf{Contextual Decomposition Algorithm} To better understand how the model handle composition of semantics to reach predictions, contextual decomposition (CD) propose to measure the contribution solely from a given phrase (or the individual contribution of the phrase) to predictions~\citep{murdoch2018beyond}. 

\xiang{compress and simplify this part. Go straight to the key technical parts that will be useful in later sections, and skip low-level details.}
We briefly introduce the line of contextual decomposition algorithms.  In the algorithm, $\phi(\rvp, \rvx^0)$ is constructed so that it represents the contribution solely from the given phrase $\rvp$. The algorithm is initially proposed for LSTM models.
Starting from the input layer, the algorithm iteratively decompose the output of each layer $\rvh$ into the contribution solely from the given phrase, noted as $\mathbf{\beta}$, and that involving other factors, noted as $\mathbf{\gamma}$, which satisfies $\rvh = \mathbf{\beta} + \mathbf{\gamma}$. For a linear layer with a word vector input $\rvx_t$, when the time step $t$ lies in the phrase we are interested in, the contribution solely from the given phrase to the output of the linear layer $\rvh=\mW_i\rvx_t+\vb_i$ is quantified as $\mathbf{\beta} = \mW_i\rvx_t$. In this case, the contribution involving other factors $\mathbf{\gamma}$ is $0$, and the contribution of the bias term $\mathbf{\zeta}$ is $b_i$ . Similarly, when the current time step $t$ lies outside the phrase, $\mathbf{\gamma}$ is quantified as $\mW_i\rvx_t$, while $\mathbf{\beta}$ is quantified as 0. 

When the algorithm encounters element-wise multiplication operations $\rvh=\rvh_a * \rvh_b$, which prevail in LSTM networks, the algorithm focuses on eliminating the multiplicative interaction terms which involve the information outside the phrase $\rvp$. Suppose that $\rvh_a$ and $\rvh_b$ have already been decomposed as $\rvh_a=\mathbf{\beta}^a + \mathbf{\gamma}^a + \zeta^a$, $\rvh_b=\mathbf{\beta}^b + \mathbf{\gamma}^b + \zeta^b$, the decomposition of the $\rvh$ is calculated as
\begin{equation}
\label{eq:cd_multiplication}
\begin{split}
    \mathbf{\beta} &= \mathbf{\beta}^a * \mathbf{\beta}^b + \mathbf{\beta}^a * \zeta^b + \zeta^a * \mathbf{\beta}^b\\
    \mathbf{\gamma}&= (\mathbf{\gamma}^a + \zeta^a) * (\mathbf{\gamma}^b + \zeta^b)
\end{split}
\end{equation}
In short, the algorithm discard the terms involving $\mathbf{\gamma}$ or only involving the bias term $\zeta$, and keeps other terms as the contribution solely from the given phrase.
%Given a sequence of words $\rvx_{1..T}$ represented in embedding vectors, LSTM iteratively updates a cell and state vector $c_t$, $h_t$.
% \begin{equation}
% \label{eq:lstm}
%     c_t, h_t = {\rm LSTM}(x_t, c_{t-1}, h_{t-1})
% \end{equation}

 
%At the initial time-step, $h_0=\mathbf{\beta}^h_0=\mathbf{\gamma}^h_0=0$ and $c_0=\mathbf{\beta}^c_0=\mathbf{\gamma}^c_0=0$. For annotations, we write the decomposed variable on the top, and the time step at the bottom of the notations. The terms involving $x_t$ updates $\mathbf{\beta}$ when current time step $t$ falls in the given phrase, or otherwise updates $\mathbf{\gamma}$. Taking the computation of $i_t=\sigma(W_ix_t + V_ih_{t-1} + b_i)$ as an example, when $t \in [i,j]$, $i_t$ is decomposed as
% \begin{equation}
% \label{eq:cd_eg}
% \begin{split}
%     i_t &= \sigma(W_ix_t + V_ih_{t-1} + b_i) \\
%         &= \sigma(\mathbf{\beta}^x_t + \mathbf{\beta}^{h}_{t-1} + \mathbf{\gamma}^{h}_{t-1} + b_i) \\
%         &= \sigma(\mathbf{\beta}^{i_x}_t + \mathbf{\gamma}^{i_x}_t + b_i)
% \end{split}
% \end{equation}
%where $W_i$ are $V_i$ the weight matrix and $b_i$ is the bias term. $h_{t-1}=\mathbf{\beta}^h_{t-1} + \mathbf{\gamma}^{h}_{t-1}$ is assumed to be decomposed in the previous time step of the algorithm. $\mathbf{\beta}^x_t$ and $\mathbf{\beta}^h_{t-1}$ terms are merged into a new term $\mathbf{\beta}_t^{i_x}$.

A main challenge is to define the decomposition for non-linear activation terms $\rvh^\prime=\sigma(\rvh)$. Contextual decomposition proposes the following decomposition to quantify the contribution solely from the phrase $\rvp$ and others.
\begin{equation}
\label{eq:cd}
\begin{split}
\mathbf{\beta}^\prime =  \frac{1}{2} [\sigma(\mathbf{\beta} + \mathbf{\gamma} + \zeta) - \sigma(\mathbf{\beta} &+ \zeta)] 
+ \frac{1}{2}[\sigma(\mathbf{\beta} + \zeta) - \sigma(\zeta)] \\
\mathbf{\gamma}^\prime = \frac{1}{2}[\sigma(\mathbf{\beta} + \mathbf{\gamma} + \zeta) - \sigma(\mathbf{\gamma} & + \zeta)]  
+ \frac{1}{2} [\sigma(\mathbf{\gamma} + \zeta) - \sigma(\zeta))] \\
\zeta^\prime = & \sigma(\zeta)
\end{split}
\end{equation}
%where $i_t=\mathbf{\beta}^i_t + \mathbf{\gamma}^i_t + \zeta^i_t$. $\zeta_t^i$ is the contribution of the bias term which is kept temporally for the element-wise multiplication in next steps. 
% Some neural models such as LSTMs involves element-wise multiplication operations. Contextual decomposition regards terms solely derive from the given phrase if they only involve $\mathbf{\beta}$ terms or the combination of $\mathbf{\beta}$ and $\zeta$ terms. Take $i_t * g_t$ as an example:
% \begin{equation}
%     \label{eq:cd_combine}
%     \begin{split}
%         i_t * g_t &= (\mathbf{\beta}^i_t + \mathbf{\gamma}^i_t + \zeta^i_t) * (\mathbf{\beta}^g_t + \mathbf{\gamma}^g_t + \zeta^g_t) \\
%         &= [\mathbf{\beta}^i_t * \mathbf{\beta}^g_t + \mathbf{\beta}^i_t * \zeta^g_t + \mathbf{\beta}^g_t * \zeta^i_t] + \mathbf{\gamma}^{i*g}_t \\
%         &= \mathbf{\beta}^{i*g}_t + \mathbf{\gamma}^{i*g}_t
%     \end{split}
% \end{equation}
The algorithm runs iteratively until it obtains the decomposition of the final output of the LSTM $\rvh_T = \mathbf{\beta}^h_T + \mathbf{\gamma}^h_T$. The logit score $\mW_l \mathbf{\beta}^h_T$ is treated as the contribution of the given phrase $\rvp$ to the final prediction.

\citet{singh2018hierarchical} extend contextual decomposition algorithms to other family of networks, and propose agglomerative contextual decomposition algorithm (ACD). The decomposition of activation functions is modified as:
\begin{equation}
    \label{eq:cd_2019}
    \begin{split}
    \mathbf{\beta}^\prime &= \sigma(\mathbf{\beta}) \\
    \mathbf{\gamma}^\prime &= \sigma(\mathbf{\beta} + \mathbf{\gamma}) - \sigma(\mathbf{\beta})
    \end{split}
\end{equation}
Besides, for the linear layer $h^\prime=Wh + b$, the bias term is decomposed proportionally and merged into $\mathbf{\beta}$ and $\mathbf{\gamma}$ terms.
\begin{equation}
    \label{eq:cd_2019_linear}
    \begin{split}
    \mathbf{\beta}^\prime &= \mW\mathbf{\beta} + \frac{|\mW\mathbf{\beta}|}{|\mW\mathbf{\beta}| + |\mW\mathbf{\gamma}|} \vb\\
    \mathbf{\gamma}^\prime &=\mW\mathbf{\gamma} + \frac{|\mW\mathbf{\gamma}|}{|\mW\mathbf{\beta}| + |\mW\mathbf{\gamma}|} \vb
    \end{split}
\end{equation}

